Extra-galactic jets: a hard X-ray view

Extragalactic jets are the most powerful persistent sources of the universe. Those pointing at us are called blazars. Their relativistically boosted emission extends from radio frequencies to TeV energies. They are also suspected to be the sources of energetic neutrinos and high energies cosmic rays. The study of their overall spectrum indicates that most of the emission of powerful blazars is in hard X-rays or in soft gamma-rays. In this band we can find the most powerful jets, visible also at high redshifts. It is found that the jet power is linked to the accretion luminosity, and exceeds it, especially if they produce energetic neutrinos, that require the presence of ultrarelativistic protons.

==> macos.tex <==
% macos.tex  (has page parameters)

\textwidth=6.2in
\textheight=8.5in
\topmargin=-.5in
\oddsidemargin=.25in
\evensidemargin=-.25in
\baselineskip=15pt plus .1pt
\def\refe{\par \noindent \hangindent=1pc \hangafter=1 }
\def\barnu{$\nu\bar\nu$~}
\def\mathnew{\mathsurround=0pt}
\def\simov#1#2{\lower .5pt\vbox{\baselineskip0pt \lineskip-.5pt
       \ialign{$\mathnew#1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
\def\simg{\mathrel{\mathpalette\simov >}}
\def\siml{\mathrel{\mathpalette\simov <}}
%\def\gtrsim{\mathrel{\mathpalette\simov >}}
%\def\lesssim{\mathrel{\mathpalette\simov <}}
\def\gele{\stackrel{>}{<}}
\def\lege{\stackrel{<}{>}}
\def\Mesz{M\'esz\'aros\,}
\def\Pacz{Paczy\'nski\,}
\def\Schr{Schr\"odinger\,}
\def\Sch{Schr\"odinger\,}
\def\Schw{Schwarzschild\,}
\def\Eot{E\"otv\"os~}
\def\U{Universe\,}
\def\ns{\normalsize}
\def\glos{\glossary}
\def\ctl{\centerline}
\def\name{name=}
\def\desc{description}
\def\dx{description}
\def\lbr{\linebreak}
\def\lbrn{\linebreak\noindent}
\def\msun{M_\odot}
\def\lsun{L_\odot}
\def\los{L.O.S.~}
\def\gr{$\gamma$-ray~}
\def\grs{$\gamma$-rays~}
\def\gamgam{$\gamma-\gamma$~}
\def\compton{\textit{Compton}\,}
\def\swift{\textit{Swift}\,}
\def\fermi{\textit{Fermi}\,}
\def\batse{\textit{BATSE}\,}
\def\gbm{\textit{GBM}\,}
\def\lat{\textit{LAT}\,}
\def\etal{{\it et~al.}\,}
\def\nonum{\nonumber}
\def\mfp{m.f.p.\,}
\def\vareps{\varepsilon}
\def\ve{\varepsilon}
\def\eps{\epsilon}
\def\lrar{\leftrightarrow}
\def\Rarrow{\Rightarrow}
\def\noind{\noindent}
\def\bull{\bullet\,}
\def\nbull{\noindent$\bullet$\,\,}
\def\nobu{\noindent$\bullet$\,\,}
\def\bitm{\bibitem}
\def\bits{\vspace{-0.3cm}\bibitem}
\def\para{\parallel}
%\def\perp{\perpendicular}
\def\beq{\begin{equation}}
\def\enq{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\ena{\end{eqnarray}}
\def\bec{\begin{center}}
\def\enc{\end{center}}
\def\bsk{\bigskip}
\def\msk{\mediumskip}
\def\ssk{\smallskip}
\def\noi{\noindent}
\def\blist{\begin{list}{$\bullet$}{\itemsep 0.0in \parsep 0.0in}}
\def\elist{\end{list}}
\def\bitem{\begin{list}{\arabic{enumi}.}{\usecounter{enumi} \itemsep 0.0in \parsep 0.0in}}
\def\eitem{\end{list}}
\def\cm{\hbox{~cm}}
\def\s{\hbox{~s}}
\def\erg{\hbox{~erg}}
\def\g{\hbox{~g}}
\def\dyne{\hbox{~dyne}}
\def\fm{\hbox{~fm}}
\def\b{{\rm b}}
\def\mb{{\rm mb}}
\def\mub{{\mu{\rm b}}}
\def\nb{{\rm nb}}
\def\pb{{\rm pb}}
\def\EeV{\hbox{EeV}}
\def\PeV{\hbox{PeV}}
\def\TeV{\hbox{~TeV}}
\def\GeV{\hbox{~GeV}}
\def\MeV{\hbox{~MeV}}
\def\keV{\hbox{~keV}}
\def\eV{\hbox{~eV}}
\def\deg{\hbox{~deg}}
\def\K{{~\hbox{K}}}
\def\Hz{\hbox{~Hz}}
\def\gmunu{g_{\mu\nu}}
\def\etamunu{\eta_{\mu\nu}}
\def\Rmunu{R_{\mu\nu}}
\def\Tmunu{T_{\mu\nu}}
\def\munu{{\mu\nu}}
\def\albet{{\alpha\beta}}
\def\pv{{\vec p}}
\def\rv{{\vec r}}
\def\vv{{\vec v}}
\def\vv{{\vec v}}
\def\uv{{\vec u}}
\def\vchi{{\vec \chi}}
\def\vr{{\vec r}}
\def\vbet{{\vec \beta}}
\def\vnab{{\vec \nabla}}
\def\xv{{\vec x}}
\def\kv{{\vec k}}
\def\qv{{\vec q}}
\def\Bv{{\vec B}}
\def\Ev{{\vec E}}
\def\Fv{{\vec F}}
\def\xp{{x'}}
\def\rph{r_{ph}}
\def\rphem{r_{ph,\gamma}}
\def\phot{photosphere~}
\def\hgamma{{\hat \gamma}}
\def\hatgam{{\hat \gamma}}
\def\gamu{\gamma^\mu}
\def\part{\partial}
%\def\partmu{\partial_\mu}
\def\bpsi{{\boldsymbol\psi}}
\def\barbpsi{{\bar{\boldsymbol\psi}}}
\def\blambda{{\boldsymbol\lambda}}
\def\bsigma{{\boldsymbol\sigma}}
\def\barnu{{\bar \nu}}
\def\barpsi{{\bar \psi}}
\def\barX{{\bar X}}
\def\barp{{\bar p}}
\def\barq{{\bar q}}
\def\barQ{{\bar Q}}
\def\barq{{\bar q}}
\def\barell{{\bar \ell}}
\def\nue{\nu_e}
\def\barnue{{\bar \nu_e}} 
\def\numu{\nu_\mu}
\def\barnumu{{\bar \nu}_\mu}
\def\nutau{\nu_\tau}
\def\barnutau{{\bar \nu}_\tau}
\def\nul{\nu_L}
\def\nur{\nu_R}
\def\er{e_R}
\def\el{e_L}
\def\psil{\psi_L}
\def\psir{\psi_R}
\def\km{{\rm km}}
\def\kg{{\rm kg}}
\def\pc{{\rm pc}}
\def\kpc{{\rm kpc}}
\def\Mpc{{\rm Mpc}}
\def\Gpc{{\rm Gpc}}
\def\sr{{\rm sr}}
\def\hr{{\rm hr}}
\def\yr{{\rm yr}}
\def\Gyr{{\rm Gyr}}
\def\Tgut{T_{GUT}}
\def\Tew{T_{EW}}
\def\mpl{m_{Pl}}
\def\m-pl{m_{Pl}}
\def\Tpl{T_{Pl}}
\def\h75{h_{75}}
\def\Omh75{\Omega h^2_{75}}
\def\Omh70{\Omega h^2_{70}}
\def\abar{{\tilde a}}
\def\aeq{a_{eq}}
\def\adec{a_{dec}}
\def\bCP{{\bf CP}}
\def\bC{{\bf C}}
\def\bP{{\bf P}}
\def\bCPT{{\bf CPT}}
\def\bB{{\bf B}}
\def\bL{{\bf L}}
\def\bT{{\rm T}}
\def\bs{\boldmath}
\def\bsy{\boldsymbol}
\def\bp{\bs{p}}
\def\bsP{\bsy{P}}
\def\cL{{\cal L}}
\def\cS{{\cal S}}
\def\calP{{\cal P}}
\def\calD{{\cal D}}
\def\calV{{\cal V}}
\def\calt{{\cal T}}
\def\tilcalD{{\tilde{\cal D}}}
\def\bA{{\bf A}}
\def\bU{{\bf U}}
\def\bD{{\bf D}}
\def\tildebD{{\tilde{\bf D}}}
\def\bA{{\bf A}}
\def\tildebA{{\tilde{\bf A}}}
\def\bF{{\bf F}}
\def\tildebF{{\tilde{\bf F}}}
\def\bH{{\bf H}}
\def\G{{\rm G}}
\def\muG{{\mu{\rm G}}}
\def\nG{{\rm nG}}

\def\fun#1#2{\lower3.6pt\vbox{\baselineskip0pt\lineskip.9pt
  \ialign{$\mathsurround=0pt#1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
%\def\lesssim{\mathrel{\mathpalette\fun <}}
%\def\gtrsim{\mathrel{\mathpalette\fun >}}
\def\VEV#1{\left\langle #1\right\rangle}
\def\sigmav{\VEV{\sigma_{\rm ann}|v|}}
\def\vectheta{\mbox{\boldmath$\theta$}}
\def\vecl{\mbox{\boldmath $l$}}

\def\jcap{Jour. Cosmology and Astro-Particle Phys.\,}
\def\mnras{M.N.R.A.S.\,}
\def\inprep{in~prep.\,}
\def\apj{Astrophys.J.\,}
\def\apjl{Astrophys.J.Lett.\,}
\def\apjs{Astrophys.J.Supp.\,}
\def\aj{Astron.J.\,}
\def\nat{Nature\,}
\def\na{New Ast.\,}
\def\nar{New~Ast.Rev.\,}
\def\nup{Nucl. Phys.\,}
\def\cmp{Comm. Math. Phys.\,}
\def\prl{Phys. Rev. Lett.\,}
\def\pl{Phys. Lett.\,}
\def\rmp{Rev. Mod. Phys.\,}
\def\ijmp{Int. Jour. Mod. Phys.\,}
\def\mpl{Mod. Phys. Lett.\,}
\def\pr{Phys. Rev.\,}
\def\prd{Phys.Rev.D\,}
\def\araa{Annu.Rev.Astron.Astrophys.\,}
\def\aap{Astron.Astrophys.\,}
\def\aaps{Astron.Astrophys.Supp.\,}
\def\aa{Astron.Astrophys.\,}
\def\pasj{Pub.Astr.Soc.Japan\,}
\def\physrep{Phys.Rep.\,}
\def\apss{Astrophys. Space Sci.}
\def\aa{\ {A\&A}\ }
\def\aap{\ {A\&A}\ }
\def\aarev{\ {A\&A Review}\ }
\def\aas{\ {A\&AS}\ }
\def\aaps{\ {A\&AS}\ }
\def\acta{\ {Acta Astron.}\ }
\def\advspres{\ {Adv. Space Res.}\ }
\def\aj{\ {AJ}\ }
\def\ajp{\ {Aust. J. Phys.}\ }
\def\ajpas{\ {Aust. J. Phys. Astr. Supp.}\ }
\def\annap{\ {Ann. d'Ap.}\ }
\def\apj{\ {ApJ}\ }
\def\apjl{\ {ApJL}\ }
\def\apjs{\ {ApJS}\ }
\def\apss{\ {Ap\&SS}\ }
\def\araa{\ {ARA\&A}\ }
\def\astrolett{\ {Astro. Lett. and Communications}\ }
\def\baas{\ {BAAS}\ }
\def\ban{\ {BAN}\ }
\def\bain{\ {Bul. Astron. Inst. Neth.}\ }
\def\cntphys{\ {Contemp. Phys.}\ }
\def\currsci{\ {Curr. Sci.}\ }
\def\jaa{\ {JA\&A}\ }
\def\jphys{\ {J. de Physique}\ }
\def\memsai{\ {Mem. Soc. Astron. Ital.}\ }
\def\mess{\ {Messenger}\ }
\def\mnras{\ {MNRAS}\ }
\def\nat{\ {Nat}\ }
\def\natps{\ {Nature Phys. Sci.}\ }
\def\newa{\ {New Astron.}\ }
\def\obs{\ {Observatory}\ }
\def\pasa{\ {Proc. Astron. Soc. Aust.}\ }
\def\pasp{\ {PASP}\ }
\def\pasj{\ {Publ. Astr. Soc. Japan}\ }
\def\pcps{\ {Proc. Cambridge Phil. Soc.}\ }
\def\pddo{\ {Pub. David Dunlap Obs.}\ }
\def\philtrans{\ {Phil. Trans. R. Soc. London A}\ }
\def\physrep{\ {PhysRep}\ }
\def\physrevl{\ {Phys. Rev. Lett.}\ }
\def\physscrip{\ {Physica Scripta}\ }
\def\phystod{\ {Physics Today}\ }
\def\pnas{\ {Proc. Nat. Acad. Sci.}\ }
\def\prd{\ {Phys. Rev. D.}\ }
\def\qjras{\ {QJRAS}\ }
\def\roa{\ {R. Obs. Annals}\ }
\def\rob{\ {R. Obs. Bull.}\ }
\def\sci{\ {Science}\ }
\def\sovast{\ {SvA}\ }
\def\ssr{\ {Space Sci. Rev.}\ }
\def\zfa{\ {Zeitschr. f. Astroph.}\ }

\def\hl{\hline}
\def\tl{\tableline}
%\newcommand{\figuresize}{0.41\textwidth}
%\newcommand{\boxsize}{0.89\textwidth}
%\newcommand{\smallboxsize}{0.8\textwidth}


